Tilted Richardson Varieties

The study of the flag variety $\mathrm{Fl}_n$ and its subvarieties, including Schubert and Richardson varieties, plays a fundamental role in algebraic geometry and algebraic combinatorics. In this paper, we introduce and develop the theory of tilted Richardson varieties $\mathrm{T}_{u,v}$, a new family of subvarieties of the flag variety that provides a geometric framework for the quantum Bruhat graphs. These varieties are defined for all pairs of permutations $u$ and $v$, extending the classical Richardson varieties in the case where $u\leq v$ in the Bruhat order. We establish their fundamental geometric properties, proving irreducibility and providing explicit dimension formulas. Moreover, we show that they have a well-defined stratification indexed by tilted Bruhat intervals, a generalization of classical Bruhat intervals previously introduced by Brenti, Fomin, and Postnikov. Additionally, we introduce a tilted generalization of the classical Deodhar decomposition of Richardson varieties, which leads to a combinatorial formula for tilted Kazhdan--Lusztig R-polynomials, a notion that arises naturally in our framework. We further develop a theory of total positivity for tilted Richardson varieties. In particular, we define and study the totally nonnegative parts of tilted Richardson varieties, proving they form a CW complex. This generalizes earlier results on the totally nonnegative flag variety and answers Bj\"orner's questions regarding geometric realizations of tilted Bruhat intervals. Finally, we establish explicit connections between tilted Richardson varieties and quantum Schubert calculus. Specifically, we prove that $\mathrm{T}_{u,v}$ coincides with minimal-degree two-point curve neighborhoods. As a result, we compute their cohomology classes and derive new relationships among Gromov--Witten invariants of the flag variety.

==> tex/9-future-work.tex <==
% Quantum Bruhat Interval Polytope
% Totally Nonegative Part (CW complex)
% Deodhar Parametrization Plucker Polynomials (combi interpretation)
% Deodhar Ansatz
% Leading Monomial of Path Schubert Polynomial
% Correct definition of Tilted Reduced Word
% Which Tuv = Txy
% Tilted Schubert Variety Xua Various Posets (Sara)
% Smoothness: Affine Richardson (tfy)
% Geometric equivalence of tilted Richardson and Affine Richardson on a chart (tfy)
% Equivariant Cohomology Class
% Quantum Hecke Algebra
% Quantum Demazure Product
% Projection: which positroid? (AK)
% Flag Positroid Variety Using Cyclic Rank? (AK)
% Two theorems for Gromov Witten Constants (cycle and pushpull)
% Frobenius Splitting (reduced ideal - AK)
% Intersection & decomposition of Schubert divisors
% Other type (vanishing loci == curve neighbourhood?)
